Stable-BC: Controlling Covariate Shift with Stable Behavior Cloning

Behavior cloning is a common imitation learning paradigm. Under behavior cloning the robot collects expert demonstrations, and then trains a policy to match the actions taken by the expert. This works well when the robot learner visits states where the expert has already demonstrated the correct action; but inevitably the robot will also encounter new states outside of its training dataset. If the robot learner takes the wrong action at these new states it could move farther from the training data, which in turn leads to increasingly incorrect actions and compounding errors. Existing works try to address this fundamental challenge by augmenting or enhancing the training data. By contrast, in our paper we develop the control theoretic properties of behavior cloned policies. Specifically, we consider the error dynamics between the system's current state and the states in the expert dataset. From the error dynamics we derive model-based and model-free conditions for stability: under these conditions the robot shapes its policy so that its current behavior converges towards example behaviors in the expert dataset. In practice, this results in Stable-BC, an easy to implement extension of standard behavior cloning that is provably robust to covariate shift. We demonstrate the effectiveness of our algorithm in simulations with interactive, nonlinear, and visual environments. We also conduct experiments where a robot arm uses Stable-BC to play air hockey. See our website here: https://collab.me.vt.edu/Stable-BC/

==> arxiv.tex <==
@inproceedings{Block2023ProvableGBC,
  title={Provable Guarantees for Generative Behavior Cloning: {B}ridging Low-Level Stability and High-Level Behavior},
  author={Adam Block and Ali Jadbabaie and Daniel Pfrommer and Max Simchowitz and Russ Tedrake},
  booktitle={Neural Information Processing Systems},
  year={2023},
  url={https://api.semanticscholar.org/CorpusID:260202777}
}

\section{Related Work}

Our work is related to papers on behavior cloning, covariate shift / compounding error, and safe imitation learning.
Original paper for behavior cloning \cite{pomerleau1988alvinn}.
Problems include covariate shift \cite{ross2010efficient, spencer2021feedback}, and possibly causal confusion \cite{de2019causal}.

\p{On-Policy} These methods seek to address covariate shift by collecting additional datapoints during task execution.
\begin{itemize}
    \item \cite{ross2011reduction} DAgger, a method for collecting new data online to improve a behavior cloned policy
    \item \cite{hoque2021thriftydagger, kelly2019hg, menda2019ensembledagger} Recent improvements to DAgger that determine when additional data is needed (human-gated, robot-gated)
    \item \cite{spencer2022expert} Improvement to DAgger that increases the information extracted from each expert intervention
\end{itemize}

\p{Off-Policy} These methods seek to address covariate shift by improving the offline dataset. This can be done as the human provides the dataset (e.g., perturbing the human teacher), or after the dataset is obtained (e.g., augmenting the dataset with synthetic datapoints).
\begin{itemize}
    \item \cite{belkhale2024data} Describes the data properties (i.e., the types of demonstrations the expert should provide) to best prevent compounding errors
    \item \cite{laskey2017dart} DART, an approach to widen the dataset distribution by injecting noise during expert demonstrations
    \item \cite{umut2024safe} Improvement to DART that injects intelligent and adversarial disturbances during expert demonstrations. This method requires information about unsafe states (i.e., the failure set)
    \item \cite{ke2023ccil, ke2021grasping, zhou2023nerf} CCIL and other methods for adding synthetic data to the dataset provided by the human (e.g., sampling nearby states and actions)
    \item \cite{chang2021mitigating} MILO uses the demonstration dataset and an additional offline dataset of rollouts to estimate the dynamics and then mitigate covariate shift
    \item \cite{hoque2024intervengen} Given a few online human corrections, this method produces a large set of synthetic corrections that mimic the human's examples.    
\end{itemize}

\p{Recovery or Filtering} These methods do not alter the dataset or directly improve the robot's learned policy. Instead, they learn a separate backup policy or safety filter to constrain the robot to in-distribution states.
\begin{itemize}
    \item \cite{reichlin2022back} Develops a recovery (i.e., backup) policy for bringing the robot back to the training states
    \item \cite{wabersich2023data, hsu2023safety} Reviews of safety filters, which modify the actions output by the policy to satisfy a known safety constraint
\end{itemize}

% https://arxiv.org/pdf/2307.14619

\p{Stability} These works are similar to our proposed method, but with different applications.
\begin{itemize}
    \item \cite{kang2022lyapunov} Limits distribution shift by extending Lyapunov stability analysis to the distribution space, which keeps the system in distribution. Applied to model-based RL (specifically, MPC).
    \item \cite{pfrommer2022tasil} TaSIL trains the behavior cloning policy such that its Taylor series terms match the Taylor series terms of an expert policy. This helps prevent covariate shift by capturing the recovery behavior of human teachers.
    \item Coupled stability (?)
    \item \cite{Totsila2023ANDPs, KhansariZadeh2011SEDS} achieve stable learned policies by imposing strict stability constraints on the learned policy class. However, the learned policies are designed to converge to a static attractor state which doesn't necessarily help with keeping the policy in distribution.
\end{itemize}


% next steps
% search again for more works
% check with SIA to complete list

\section{Problem Statement}

We consider settings where a robot is using behavior cloning to imitate a human.
This includes settings where the robot is acting in isolation (e.g., a robot arm reaching a goal position), as well as interactive tasks where the robot must reason over other agents (e.g., an autonomous car at an intersection with human drivers).
Offline the robot is provided with a dataset of state-action pairs, and the robot uses behavior cloning to train a policy that matches this dataset.
Our objective is for the robot to \textit{safely extrapolate} from the dataset to the learned policy, so that online --- when the robot rolls outs this policy --- the system is robust to covariate shift and out-of-distribution data.

% this work is more about staying in distribution (avoiding covariate shift) than it is about "safety"


\p{Robot}
The robot's state is $x$ and the robot's action is $u$. 
The robot's state transitions according to the dynamics: $\dot{x}(t) = f\big(x(t), u(t)\big)$.
We assume that the robot's state and dynamics are known.

\p{Environment}
The robot interacts with an environment.
This environment could contain static goals, dynamic objects, or even other agents.
We write the state of the environment as $y$ with dynamics: $\dot{y}(t) = g\big(y(t), x(t))$.
We assume that the robot can observe the environment state $y$, but we do not assume that the robot knows the environmental dynamics $g$.

\p{Dataset} 
The robot is given a dataset $\mathcal{D}$ of $n$ state-action pairs. The overall system state $(x, y)$ consists of both the robot's state and the environment state. Hence, the offline dataset is: $\mathcal{D} = \{(x_1, y_1, u_1), \ldots, (x_n, y_n, u_n)\}$.

\p{Objective} 
Given only the robot dynamics $f$, the observations $x$ and $y$, and the dataset $\mathcal{D}$, we seek to learn a robot policy $\pi : \mathcal{X} \times \mathcal{Y} \rightarrow \mathcal{U}$ that is robust to covariate shift and states the robot has not been trained on.

\section{Method}

Our core hypothesis is that: \textit{robots are safe when they stick to what they know}. 
Let $(x', y') \notin \mathcal{D}$ be the system's current state, and let $(x, y) \in \mathcal{D}$ be a labeled state where the robot knows exactly what action to take.
Within this context, our hypothesis suggests that robust robots should take actions that move from the unlabeled state $(x', y')$ towards labeled states $(x, y)$.
Below we leverage this insight to enhance the robustness of standard behavior cloning algorithms.

% We can address this distribution shift problem by minimizing the mismatch between state visitation
% distribution of a learned policy π and the state visitation distribution of an demonstration policy πE

\p{Stability Analysis} 
Our analysis starts by considering the covariance shift between nearby states $(x', y')$ and $(x, y)$:
\begin{equation}
    \dot{x}' - \dot{x} = f(x', u') - f(x, u)
\end{equation}
\begin{equation}
    \dot{y}' - \dot{y} = g(y', x') - g(y, x)
\end{equation}
Substituting in $u = \pi(x,y)$ and using a first-order Taylor series approximation, we can rewrite the covariance shift as:
\begin{equation}
    \dot{x}' - \dot{x} = \Big(\nabla_x f + \nabla_u f \cdot \nabla_x \pi \Big) (x' - x) + \Big(\nabla_u f \cdot \nabla_y \pi \Big) (y' - y)
\end{equation}
\begin{equation}
    \dot{y}' - \dot{y} = \nabla_y g \cdot (y' - y) + \nabla_x g \cdot (x' - x)
\end{equation}
In the above, all gradients are taken about the labeled state $(x, y)$.
We can express these coupled equations in standard form:
\begin{equation}
    \dot{z} = Az
\end{equation}
\begin{equation} \label{eq:A}
    z = 
    \begin{bmatrix}
        x' - x \\
        y' - y
    \end{bmatrix}, \quad A = 
    \begin{bmatrix}
        \nabla_x f + \nabla_u f \cdot \nabla_x \pi & \nabla_u f \cdot \nabla_y \pi \\
        \nabla_x g & \nabla_y g
    \end{bmatrix}
\end{equation}
We conclude that the covariance shift locally converges towards zero if the matrix $A$ is stable (i.e., all eigenvalues of $A$ have negative real parts).

\p{Rate of Convergence} The system locally converges to an equilibrium $(x, y)$ from the dataset in an exponential manner \cite{teschl2012ordinary} (Theorem 6.10). 
The rate of convergence is determined by the eigenvalues of $A$, where increasingly negative eigenvalues mean faster convergence to the local equilibrium.

\p{Stability and Performance} Training the robot's policy $\pi$ so that $A$ is stable ensures that the system locally converges towards labeled states $(x,y)$. 
Each point in the dataset effectively becomes a basin of attraction, and --- if we train the robot's policy to only stabilize $A$ --- the system will come to rest after reaching some $(x,y)$.
We note that this stability can conflict with task performance.
If the system needs to reach some new state $(x', y')$ to complete the task, and every labeled state $(x,y)$ is truly stable, then at best the system will converge to a labeled state $(x,y)$ that is near $(x', y')$.
Hence, for a performant robot policy, we \textit{may not want} every state in the environment to be stable.

\p{Loss Function} In practice, we resolve this theoretical conflict between stability and performance by training the robot to match the human's demonstrations (standard behavior cloning loss) while also penalizing non-stable matrices $A$ (our proposed addition).
Our loss function is:
\begin{equation} \label{eq:loss}
    \mathcal{L}(\pi) = \sum_{(x, y, u) \in \mathcal{D}} \Bigg[ \| u - \pi(x, y) \|^2 + \lambda \sum_{\sigma_i \in \text{eig}(A)} \text{ReLU}\big(\text{Re}(\sigma_i)\big) \Bigg]
\end{equation}

\p{Impact} We can mitigate covariate shift in behavior cloned policies by training $\pi(x, y)$ so that (standard loss function) the policy matches the dataset $\mathcal{D}$ and (added loss term) the matrix $A$ is stable at states $(x, y) \in \mathcal{D}$.


\subsection{Model Based}

We first consider settings where $g$ is known by the robot (i.e., the robot is given a model of the environment).
In these model-based scenarios the robot full has access to matrix $A$ from \eq{A}.
Here we can directly apply \eq{loss} to train the robot's policy.


\subsection{Model Free}

We next consider settings where $g$ is unknown (i.e., the robot does not have a model of the environment).
In these model-free settings the robot only knows the first row of matrix $A$ from \eq{A}.

\p{General Case} If we know nothing about $g$ or $y'$, then we cannot make any guarantees about the overall stability of $A$.


%%% check: Bellman Gronwell Lemma

\p{Bounded Environmental Shift} In many settings it may be reasonable to assume that the environment behavior at training time is similar to the environment behavior at test time.
This implies that $\| y' - y \|$ has an upper bound.
Assume $\| y' - y\| < \epsilon$, and choose $\pi$ such that $\nabla_x f + \nabla_u f \cdot \nabla_x \pi$ is stable.
If $\lambda_{min}$ is the is a lower bound on the magnitude of $\nabla_x f + \nabla_u f \cdot \nabla_x \pi$, then $\|x' - x\|$ is uniformly ultimately bounded with radius:
\begin{equation}
    \| x' - x \| \leq \frac{1}{\lambda_{min}} \cdot \| \nabla_u f \cdot \nabla_y \pi \| \cdot \epsilon, \quad \lambda_{min} = \frac{1}{\|(\nabla_x f + \nabla_u f \cdot \nabla_x \pi)^{-1}\|}
\end{equation}
This suggests the following:
\begin{itemize}
    \item We should choose $\pi$ such that $\nabla_x f + \nabla_u f \cdot \nabla_x \pi$ is stable
    \item We should choose $\pi$ to regulate the magnitude $\| \nabla_u f \cdot \nabla_y \pi \|$ 
\end{itemize}
However, we emphasize that if $\| \nabla_u f \cdot \nabla_y \pi \| = 0$, the robot's policy no longer depends on $y$.
This is another example of the conflict between stability and performance: in most cases the robot should take the environment state into account when making decisions.
Hence, we must carefully trade-off between regulating $\| \nabla_u f \cdot \nabla_y \pi \|$ and ensuring the robot matches the human's examples. 
With this analysis in mind, we propose the following loss function for model free scenarios where we can assume $\|y' - y\|$ is bounded:
\begin{equation} \label{eq:loss}
    \mathcal{L}(\pi) = \sum_{(x, y, u) \in \mathcal{D}} \Bigg[ \| u - \pi(x, y) \|^2 + \lambda_1 \|A_y\| + \lambda_2 \sum_{\sigma_i \in \text{eig}(A_x)} \text{ReLU}\big(\text{Re}(\sigma_i)\big) \Bigg]
\end{equation}
\begin{equation}
    A_x = \nabla_x f + \nabla_u f \cdot \nabla_x \pi, \quad A_y = \nabla_u f \cdot \nabla_y \pi
\end{equation}
The only difference between this loss function and \eq{loss} is that here we also regulate the magnitude of the term $A_y$.

\section{Simulations}% \label{sec:sims}

There are two simulated environments we are currently planning for the paper:
\begin{enumerate}
    \item (Collab) A linear intersection environment where a human and autonomous car are crossing paths. The simulation can be visualized in CARLO. The human's policy depends on $x$ and $y$.
    \item (SIA) A nonlinear aircraft landing environment. At first the simulation will have a static goal ($g = 0$), but this could be changed later. Will include state-based and vision-based states.
\end{enumerate}

\section{User Study}% \label{sec:userstudy}

We are planning one user study for the paper.
This study will take place with a Franka robot arm and a human user.
The human and robot are interacting to play air hockey (?)
